Approaching the isoperimetric problem in $H^m_{\mathbb{C}}$ via the hyperbolic log-convex density conjecture

We prove that geodesic balls centered at some base point are isoperimetric in the real hyperbolic space $H_{\mathbb R}^n$ endowed with a smooth, radial, strictly log-convex density on the volume and perimeter. This is an analogue of the result by G. R. Chambers for log-convex densities on $\mathbb R^n$. As an application we prove that in any rank one symmetric space of non-compact type, geodesic balls are isoperimetric in a class of sets enjoying a suitable notion of radial symmetry.

==> hopf_sets.tex <==
\subsection{Setting}We consider $(M^n,g)=(H_{\K}^m,g)$ to be a rank one symmetric space of non compact type, $\K\in\{\C,\Ham,\Oct\}$. Fix an arbitrary base point $o\in M$, and consider $(T_oM,\exp_o^*g)=:(\R^n,g)$ the exponential lift to an arbitrary tangent space. The following lemma allows us to compute surfaces in normal coordinates.
\begin{lemma}\label{lem:general_formula}
Let $\Sigma$ be an oriented $C^1$-hypersurface of $(\R^n,g)$, where $g$ denotes any Riemannian metric. Then the area of $\Sigma$ is given by
\[
A(\Sigma)=\int_\Sigma\sqrt{\abs{g}}g_{\text{flat}}(g^{-1}n,n)^{1/2}\,d\Haus^{n-1},
\]
where $n$ denotes the Euclidean normal vector field of $\Sigma$.
\end{lemma}
\begin{proof}Let $\nu$ be the normal vector field of $\Sigma$ with respect to $g$. 
Fix $x\in\Sigma$, and let $v_1,\dots,v_{n-1}$ be a basis of $T_x\Sigma$. Then, $\nu$ is uniquely (up to orientation) determined by the conditions $g(\nu,\nu)=1$ and $g(\nu,v_j)=0$ for $j=1,\dots,n-1$. Therefore, we get the identity $\nu=g(g^{-1}n,g^{-1}n)^{-1/2}g^{-1}n$. Finally,
\begin{align*}
A(\Sigma)&=\int_{\Sigma}\iota_{\nu}\vol=\int_{\Sigma}\sqrt{\abs{g}}\iota_{\nu}\,dx=\int_{\Sigma}\sqrt{\abs{g}}\inn{g^{-1}n,n}^{-1/2}\iota_{g^{-1}n}\,dx\\
&=\int_{\Sigma}\sqrt{\abs{g}}\inn{g^{-1}n,n}^{-1/2}\inn{g^{-1}n,n}\iota_{n}\,dx=\int_\Sigma\sqrt{\abs{g}}\inn{g^{-1}n,n}^{1/2}\,d\Haus^{n-1}.
\end{align*}
\end{proof}
As in Definition \ref{def:hopf_symmetric}, let $\Dist$ be the distribution induced by the $(-4)$-eigenspace of the Jacobi operator $R(n,\cdot)n$ and denote with $\Vist$ the $(m-1)\dim(\K)$ dimensional distribution associated to its $(-1)$-eigenspace, so that at every point $x\in M\setminus\{o\}$, the tangent space $T_xM$ decomposes as a direct sum of mutual orthogonal subspaces $T_xM=\Dist_x\oplus\Vist_x\oplus\R x$.
\iffalse
We lift $M$ on an arbitrary tangent space $T_oM$ by mean of the exponential map. For any direction $x\in T_oM$ we call $r=\abs{x}$ the norm of $x$. Set $\frac xr=v_0\in T_oM$ and $v_i=J_iv_0$ for $i=1,\dots,d-1$. Complete the orthonormal basis with the vectors $v_d,\dots,v_{n-1}$. With $v_i(r)$ we denote the parallel transport of $v_i$ along the geodesic $r\mapsto\exp_o(rv_0)$, so that the Jacobi fields $Y_i(r)$ with initial conditions $Y_i(0)=0,\,Y_i'(0)=v_i$ are given by
\[
Y_i(r)=f_i(r)v_i(r),\quad \text{where }f_i(r)=\begin{cases}r,&\text{ if }i=0,\\
\sinh(r)\cosh(r),&\text{ if }i=1,\dots,d-1,\\ \sinh(r),&\text{ if }i=d,\dots,n-1.\end{cases}
\]
Then, the pullback metric $\exp_o^* g$ (that by abuse of notation we will still denote with $g$ since $(T_oM,\exp_o^* g)$ and $(M,g)$ are isometric) is given in the basis $\{v_0,\dots,v_{n-1}\}$ by the diagonal matrix
\[
(\exp^*_og)_{x}(v_i,v_j)=g(d\exp_o(rv_0)[v_i],d\exp_o(rx)[v_j])=\frac {1}{r^2} g(Y_i(r),Y_j(r))=\frac{f^2_i(r)}{r^2}\delta_{ij}.
\]
The associated volume form has density
\[
\omega(r):=\sqrt{\abs{g_{x}}}=\frac{\sinh^{n-1}(r)\cosh^{d-1}(r)}{r^{n-1}}.
\]
\subsection{A change of variable in Poincaré coordinates}Let $F:B(0,1)\to (\R^n,g)$ be defined as $F(x)=2\arctanh(r)\frac xr$. Then, the pullback metric on $B(0,1)$ with respect to the same frame $v_0,\dots,v_{n-1}$ is given by
\[
(F^*g)_x(v_i,v_j)=g_{F(x)}(F_*v_i,F_*v_j).
\]
Now,
\[
F_*v_i=\begin{cases}
\frac{2}{1-r^2}v_0,&\text{ if }i=0,\\
\frac{2\arctanh(r)}{r}v_i,&\text{ if }i=1,\dots,n-1,
\end{cases}
\]
and
\[
(g_{F(x)})_{ii}=\begin{cases}
1,&\text{ if } i=0,\\
\Bigl(\frac{2r}{1-r^2}\Bigr)^2\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^2/(2\arctanh(r))^2,&\text{ if }i=1,\dots,d-1,\\
\Bigl(\frac{2r}{1-r^2}\Bigr)^2/(2\arctanh(r))^2,&\text{ if }i=d,\dots,n-1,
\end{cases}
\]
imply that
\[
(F^*g)_{ii}=\frac{4}{(1-r^2)^2}\begin{cases}1,&\text{ if }i=0,\\
\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^2,&\text{ if }i=1,\dots,d-1,\\
1,&\text{ if }i=d,\dots,n-1.\\
\end{cases}
\]
We can now apply Lemma \ref{lem:general_formula} to obtain that for any smooth subset $E\subset B(0,1)$, the perimeter with respect to $F^*g$ can be computed as
\begin{equation}\label{eq:perim}
P(E)=\int_{\partial E}\Bigl(\frac{2}{1-r^2}\Bigr)^{n-1}\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^{d-1}\Bigl(1-\frac{4r^2}{(1+r^2)^2}\sum_{i=1}^{d-1}g_{\text{flat}}(n,v_i)^2\Bigr)^{1/2}\,d\Haus^{n-1},
\end{equation}
and the volume as
\begin{equation}\label{eq:vol}
V(E)=\int_E \Bigl(\frac{2}{1-r^2}\Bigr)^{n}\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^{d-1}\,d\Haus^n.
\end{equation}
We can now prove Theorem \ref{thm:2}.
\begin{proof}[Proof of Theorem \ref{thm:2}]Looking at Equations \eqref{eq:perim} and \eqref{eq:vol}, we notice that the measures
\[
\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^{d-1}\Bigl(\frac{2}{1-r^2}\Bigr)^{n-1}d\Haus^{n-1},
\]
and
\[
\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^{d-1}\Bigl(\frac{2}{1-r^2}\Bigr)^{n}d\Haus^{n},
\]
are nothing else than the perimeter and volume measures in $H^n_{\R}$ weighted by
\[
f(r)=\Bigl(\frac{1+r^2}{1-r^2}\Bigr)^{d-1}.
\]
Assuming $E$ Hopf-symmetric, the anisotropic term
\[
\Bigl(1-\frac{4r^2}{(1+r^2)^2}\sum_{i=1}^{d-1}g_{\text{flat}}(n,v_i)^2\Bigr)^{1/2}=1.
\]
We need check that
\[
s\mapsto \ln(f\circ\tanh(s/2))=(d-1)\ln(\cosh(s)),
\]
is strictly convex. This is the case  since $\frac{d^2}{ds^2}\ln(\cosh(s))=\sech^2(s)>0$.
\end{proof}
\fi
